The Managerial Effects of Algorithmic Fairness Activism

How do ethical arguments affect AI adoption in business? We randomly expose business decision-makers to arguments used in AI fairness activism. Arguments emphasizing the inescapability of algorithmic bias lead managers to abandon AI for manual review by humans and report greater expectations about lawsuits and negative PR. These effects persist even when AI lowers gender and racial disparities and when engineering investments to address AI fairness are feasible. Emphasis on status quo comparisons yields opposite effects. We also measure the effects of "scientific veneer" in AI ethics arguments. Scientific veneer changes managerial behavior but does not asymmetrically benefit favorable (versus critical) AI activism.

==> Algorithmic Fairness Rhetoric/Tables/Descriptives.tex <==
\begin{tabular}{l*{14}{c}}
                    &       Op-Ed&      Veneer\\
\hline
Male                &        0.49&        0.52\\
Female              &        0.49&        0.45\\
Other Gender        &        0.02&        0.02\\
Latinx              &        0.10&        0.07\\
White               &        0.81&        0.85\\
Black               &        0.07&        0.05\\
Asian               &        0.05&        0.04\\
Other Ethnicity     &        0.06&        0.06\\
AI Decisions        &        0.49&        0.40\\
Prepared by Educ.   &        0.75&        0.71\\
Knows ML            &        0.46&        0.45\\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/FairnessRhetoric-Table.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Damage Size}\\
\hline
Hiring              &       -.088   &       -.055   &     2.0e-17   &        -.04   &        -.28***\\
                    &      (.082)   &      (.085)   &         (.)   &      (.087)   &      (.079)   \\
Algorithm Fix       &         .37***&         .27***&        .019   &        -.61***&        -.28***\\
                    &       (.04)   &      (.034)   &      (.034)   &      (.045)   &      (.034)   \\
Counterfactual Op-Ed&         .24** &         .19*  &         .14** &        -.12   &        -.14   \\
                    &       (.11)   &       (.11)   &      (.054)   &       (.12)   &       (.11)   \\
AI Fatalism Op-Ed   &        -.16   &        -.28***&       -.079   &         .19*  &        .061   \\
                    &       (.11)   &       (.11)   &      (.063)   &       (.11)   &      (.094)   \\
Fix$\times$ Counterfactual&       -.042   &      -.0064   &        -.28** &         .16*  &        .041   \\
                    &      (.078)   &      (.061)   &       (.11)   &      (.086)   &      (.075)   \\
Fix$\times$ AI Fatalism&       -.044   &        .012   &         .16   &          .1   &        .012   \\
                    &      (.075)   &      (.062)   &       (.13)   &      (.077)   &      (.058)   \\
\hline
Fixed Effects       &     Subject   &     Subject   &     Subject   &     Subject   &     Subject   \\
Observations        &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   \\
\(R^{2}\)           &         .68   &         .72   &         .76   &         .63   &         .73   \\
$p$-value: Counterfactual (CF)=Fatalism (FAT)&      .00061   &      .00003   &      .00079   &       .0057   &        .051   \\
\hline $p$-value: Fix$\times$CF=Fix$\times$FAT&         .98   &         .82   &      .00079   &         .59   &         .74   \\
$p$-value: CF+Fix$\times$CF=FAT+Fix$\times$FAT&      .00016   &     .000021   &      .00079   &        .031   &         .11   \\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/FairnessRhetoric-Table2.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Damage Size}\\
\hline
Algorithm Fix       &         .47***&         .45***&     1.3e-14   &         -.7***&        -.34***\\
                    &      (.057)   &      (.051)   &         (.)   &      (.061)   &      (.044)   \\
Status Quo Shown    &         .52***&         .65***&         .57***&        -.43***&        -.44***\\
                    &        (.1)   &        (.1)   &      (.094)   &      (.095)   &      (.099)   \\
Status Quo Shown (only if clicked)&         .46***&         .63***&         .54***&        -.38***&        -.42***\\
                    &       (.11)   &      (.099)   &      (.096)   &      (.092)   &      (.098)   \\
Fix $\times$ Status Quo Shown&        -.17** &        -.26***&    -2.2e-14   &         .19** &         .12*  \\
                    &      (.072)   &      (.063)   &         (.)   &      (.084)   &      (.061)   \\
Fix $\times$  Status Quo Shown (only if clicked)&        -.19** &         -.3***&    -1.9e-14   &          .2** &        .091   \\
                    &      (.076)   &      (.062)   &         (.)   &      (.082)   &      (.061)   \\
Female              &        -.16** &        -.11   &        -.15** &         .11   &         .29***\\
                    &       (.07)   &      (.072)   &      (.071)   &      (.066)   &      (.071)   \\
Black               &        -.25*  &        -.22*  &       -.048   &         .18   &         .22*  \\
                    &       (.14)   &       (.13)   &       (.13)   &       (.11)   &       (.13)   \\
Asian               &        -.17   &       -.027   &       -.084   &       -.026   &        -.16   \\
                    &       (.13)   &       (.13)   &       (.16)   &       (.14)   &       (.15)   \\
Other Ethnicity     &        -.33***&        -.26*  &        -.21   &        .083   &       -.086   \\
                    &       (.12)   &       (.14)   &       (.16)   &       (.14)   &       (.15)   \\
Political Conservatism (Standardized)&        .094** &        .082** &        .026   &       -.067** &       -.079** \\
                    &      (.038)   &      (.037)   &      (.036)   &      (.034)   &      (.038)   \\
AI Decisions        &         .12*  &         .12*  &        .078   &        .025   &        .019   \\
                    &      (.069)   &      (.072)   &      (.075)   &      (.067)   &      (.074)   \\
Prepared by Educ.   &         .13   &         .14*  &        .099   &        -.12*  &        -.12   \\
                    &       (.08)   &      (.083)   &      (.082)   &      (.075)   &       (.08)   \\
Knows ML            &       .0055   &       .0028   &       -.056   &        .062   &       -.097   \\
                    &       (.07)   &      (.074)   &      (.074)   &      (.068)   &      (.076)   \\
\hline
Observations        &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   \\
\(R^{2}\)           &          .1   &         .12   &         .12   &         .12   &        .097   \\
\hline $p$-value: Status Quo (SQ) Shown + Fix $\times$ SQ Shown=0&       .0005   &      .00018   &     2.4e-09   &        .024   &       .0023   \\
$p$-value: SQ Optional + Fix $\times$ SQ Opt=0&       .0075   &       .0018   &     3.0e-08   &        .097   &       .0017   \\
\hline $p$-value: SQ Shown = SQ Opt&         .48   &         .85   &         .74   &         .57   &         .85   \\
$p$-value: Fix $\times$ SQ Shown = Fix $\times$ SQ Opt&         .75   &         .37   &           1   &         .86   &         .69   \\
$p$-value: SQ Shown+Fix $\times$ SQ Shown = SQ Opt+Fix $\times$ SQ Opt&         .32   &         .47   &         .74   &          .5   &         .95   \\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/ScientificVeneer-Table.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Damage Size}\\
\hline
Hiring              &        -.13   &        -.23** &    -1.3e-17   &       .0022   &        -.17*  \\
                    &      (.096)   &      (.094)   &         (.)   &      (.091)   &      (.093)   \\
Algorithm Fix       &         .35***&         .27***&        .049   &        -.52***&        -.24***\\
                    &       (.04)   &      (.036)   &      (.044)   &      (.043)   &      (.036)   \\
Scientific Veneer   &        .036   &        .093   &        -.21***&        -.17   &       -.036   \\
                    &       (.16)   &       (.15)   &      (.079)   &       (.15)   &       (.13)   \\
Pro-AI Argument     &         1.1***&         1.1***&         .17** &        -.86***&        -.48***\\
                    &       (.13)   &       (.14)   &      (.071)   &       (.14)   &       (.13)   \\
Scientific Veneer $\times$ Pro AI&       -.019   &       -.072   &         .27** &         .24   &       -.037   \\
                    &       (.21)   &        (.2)   &       (.11)   &       (.21)   &       (.19)   \\
Fix $\times$ Scientific Veneer&        .078   &       -.046   &         .43***&       .0013   &      -.0084   \\
                    &        (.1)   &       (.08)   &       (.16)   &        (.1)   &       (.07)   \\
Fix $\times$ Pro-AI &        -.29***&        -.28***&        -.34** &         .24** &        .033   \\
                    &      (.073)   &      (.062)   &       (.14)   &       (.11)   &       (.07)   \\
Fix $\times$ Scientific Veneer $\times$ Pro-AI&       -.084   &         .23*  &        -.54** &        .049   &          .1   \\
                    &       (.14)   &       (.12)   &       (.23)   &       (.16)   &       (.11)   \\
\hline
Fixed Effects       &     Subject   &     Subject   &     Subject   &     Subject   &     Subject   \\
Observations        &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   \\
\(R^{2}\)           &         .62   &         .67   &         .63   &         .62   &         .69   \\
\hline $p$-value: Veneer (Ven) +Ven$\times$ProAI = 0&          .9   &         .87   &         .49   &         .66   &         .58   \\
$p$-value: Ven$\times$Fix +Ven$\times$ProAI$\times$Fix = 0&         .96   &        .027   &         .49   &         .69   &         .29   \\
$p$-value: Ven+Ven$\times$Fix +Ven$\times$ProAI+Ven$\times$ProAI$\times$Fix = 0&         .93   &         .11   &         .49   &         .36   &         .89   \\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/ScientificVeneer-Table2.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Damage Size}\\
\hline
Algorithm Fix       &         .34***&         .32***&    -2.9e-15   &        -.51***&        -.23***\\
                    &      (.055)   &      (.047)   &   (2.9e-09)   &      (.057)   &      (.042)   \\
Status Quo Shown    &         .35***&         .55***&         .51***&        -.21** &        -.16*  \\
                    &      (.086)   &      (.086)   &      (.081)   &      (.085)   &      (.086)   \\
Status Quo Shown (only if clicked)&         .28***&         .57***&         .57***&        -.27***&        -.21** \\
                    &      (.088)   &      (.087)   &       (.08)   &      (.084)   &      (.092)   \\
Fix $\times$ Status Quo Shown&        -.11   &        -.16** &     3.0e-15   &        .087   &         .03   \\
                    &      (.072)   &      (.064)   &   (2.3e-09)   &      (.079)   &      (.056)   \\
Fix $\times$  Status Quo Shown (only if clicked)&       -.043   &        -.14** &     5.5e-15***&        .089   &        .023   \\
                    &      (.074)   &      (.062)   &   (1.5e-15)   &      (.078)   &      (.062)   \\
Female              &        -.05   &       -.016   &       -.034   &       .0037   &          .1   \\
                    &      (.063)   &      (.067)   &      (.067)   &      (.066)   &      (.075)   \\
Black               &        -.55***&        -.42***&        -.28** &       -.032   &       -.048   \\
                    &       (.11)   &       (.12)   &       (.12)   &       (.17)   &       (.19)   \\
Asian               &        -.17   &        -.12   &         -.2   &       -.053   &         .21*  \\
                    &       (.11)   &       (.12)   &       (.15)   &       (.14)   &       (.12)   \\
Other Ethnicity     &        -.53***&        -.43** &        -.19   &          .2   &         .14   \\
                    &       (.15)   &       (.17)   &       (.15)   &       (.15)   &       (.18)   \\
Political Conservatism (Standardized)&         .16***&         .13***&        .091***&        -.15***&        -.14***\\
                    &      (.032)   &      (.033)   &      (.034)   &      (.033)   &       (.04)   \\
AI Decisions        &        .019   &      -.0022   &       -.058   &      -.0055   &       -.028   \\
                    &      (.064)   &      (.067)   &      (.069)   &      (.068)   &      (.077)   \\
Prepared by Educ.   &         .17***&         .08   &        .062   &         -.2***&        -.16** \\
                    &      (.064)   &      (.068)   &      (.073)   &      (.067)   &      (.077)   \\
Knows ML            &         .12*  &         .15** &         .13*  &       -.027   &       -.098   \\
                    &      (.065)   &      (.067)   &      (.068)   &      (.069)   &      (.078)   \\
\hline
Observations        &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   \\
\(R^{2}\)           &         .11   &         .11   &        .086   &        .094   &        .063   \\
\hline $p$-value: Status Quo (SQ) Shown + Fix $\times$ SQ Shown=0&       .0038   &     8.7e-06   &     9.4e-10   &         .19   &         .16   \\
$p$-value: SQ Optional + Fix $\times$ SQ Opt=0&       .0032   &     5.5e-07   &     3.5e-12   &        .043   &        .058   \\
\hline $p$-value: SQ Shown = SQ Opt&         .41   &         .81   &          .4   &         .45   &         .55   \\
$p$-value: Fix $\times$ SQ Shown = Fix $\times$ SQ Opt&         .31   &         .76   &           1   &         .98   &         .91   \\
$p$-value: SQ Shown+Fix $\times$ SQ Shown = SQ Opt+Fix $\times$ SQ Opt&         .99   &         .63   &          .4   &         .48   &         .53   \\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/StatusQuoOpEd-iv.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Damage Size}\\
\hline
Status Quo Seen (Instrumented by Op-Ed)&         1.2***&         .69***&        -.84***&        -.35*  \\
                    &       (.28)   &        (.2)   &       (.32)   &       (.21)   \\
\hline
Instrument          &    CF Op-Ed   &   FAT Op-Ed   &    CF Op-Ed   &   FAT Op-Ed   \\
Observations        &       1,992   &       1,992   &       1,992   &       1,992   \\
1st Stage F-Stat    &          86   &         187   &          86   &         187   \\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/StatusQuoOpEd.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Views Status Quo}\\
\hline
Fatalism            &        -.31   &               &        -.37   &               &        -.16   &               &         .31   &               &         .38   &               &        -.17   \\
                    &       (.27)   &               &       (.27)   &               &       (.24)   &               &       (.26)   &               &        (.3)   &               &       (.18)   \\
Counterfactual      &               &         .26   &               &         .32   &               &         .14   &               &        -.27   &               &        -.32   &        .044   \\
                    &               &       (.23)   &               &       (.22)   &               &        (.2)   &               &       (.22)   &               &       (.25)   &       (.16)   \\
\hline
Observations        &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &         996   \\
\(R^{2}\)           &        .038   &        .069   &        .071   &          .1   &         .12   &         .13   &        .076   &          .1   &       .0065   &        .044   &         .94   \\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/StatusQuoScientific-iv.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Damage Size}\\
\hline
Status Quo Seen (Instrumented by Veneer Treatment)&        -.35   &        -1.1   &        -.05   &         4.5   \\
                    &       (.68)   &       (3.8)   &       (.69)   &       (6.8)   \\
\hline
Perspective         &     Anti-AI   &      Pro-AI   &     Anti-AI   &      Pro-AI   \\
Observations        &       1,984   &       1,984   &       1,984   &       1,984   \\
1st Stage F-Stat    &          12   &          .6   &          12   &          .6   \\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/StatusQuoScientific.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Views Status Quo}\\
\hline
Scientific Veneer   &               &        -.22   &               &       -.035   &               &        -.27   &               &         1.4   &               &         1.3   &        -.25   \\
                    &               &       (1.2)   &               &       (1.2)   &               &       (1.5)   &               &       (2.2)   &               &       (2.2)   &       (.35)   \\
Pro-AI Argument     &               &               &               &               &               &               &               &               &               &               &        -.35   \\
                    &               &               &               &               &               &               &               &               &               &               &       (.29)   \\
Scientific Veneer $\times$ Pro AI&               &               &               &               &               &               &               &               &               &               &         .29   \\
                    &               &               &               &               &               &               &               &               &               &               &       (.53)   \\
\hline
Observations        &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &         992   \\
\(R^{2}\)           &        .015   &        .024   &       .0034   &        .047   &        -.12   &        -.39   &        .041   &        -1.1   &        .016   &        -1.1   &         .84   \\
\end{tabular}


==> Algorithmic Fairness Rhetoric/Tables/StatusQuoScientific2.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Views Status Quo}\\
\hline
Scientific Veneer   &        -.39   \\
                    &       (.26)   \\
Pro-AI Argument     &        -.45*  \\
                    &       (.26)   \\
Scientific Veneer $\times$ Pro AI&         .77*  \\
                    &       (.43)   \\
\hline
Observations        &         334   \\
\(R^{2}\)           &        .013   \\
\end{tabular}


==> Tables/StatusQuoOpEd.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Views Status Quo}\\
\hline
Fatalism            &        -.31   &               &        -.37   &               &        -.16   &               &         .31   &               &         .38   &               &        -.17   \\
                    &       (.27)   &               &       (.27)   &               &       (.24)   &               &       (.26)   &               &        (.3)   &               &       (.18)   \\
Counterfactual      &               &         .26   &               &         .32   &               &         .14   &               &        -.27   &               &        -.32   &        .044   \\
                    &               &       (.23)   &               &       (.22)   &               &        (.2)   &               &       (.22)   &               &       (.25)   &       (.16)   \\
\hline
Observations        &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &       1,992   &         996   \\
\(R^{2}\)           &        .038   &        .069   &        .071   &          .1   &         .12   &         .13   &        .076   &          .1   &       .0065   &        .044   &         .94   \\
\end{tabular}


==> Tables/StatusQuoScientific-iv.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Damage Size}\\
\hline
Status Quo Seen (Instrumented by Veneer Treatment)&        -.35   &        -1.1   &        -.05   &         4.5   \\
                    &       (.68)   &       (3.8)   &       (.69)   &       (6.8)   \\
\hline
Perspective         &     Anti-AI   &      Pro-AI   &     Anti-AI   &      Pro-AI   \\
Observations        &       1,984   &       1,984   &       1,984   &       1,984   \\
1st Stage F-Stat    &          12   &          .6   &          12   &          .6   \\
\end{tabular}


==> Tables/StatusQuoScientific.tex <==
\begin{tabular}{l*{14}{c}}
                    &\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Positive}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Scale)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Rec (Y/N)}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Lawsuit}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Damage Size}&\multicolumn{1}{c}{Views Status Quo}\\
\hline
Scientific Veneer   &               &        -.22   &               &       -.035   &               &        -.27   &               &         1.4   &               &         1.3   &        -.25   \\
                    &               &       (1.2)   &               &       (1.2)   &               &       (1.5)   &               &       (2.2)   &               &       (2.2)   &       (.35)   \\
Pro-AI Argument     &               &               &               &               &               &               &               &               &               &               &        -.35   \\
                    &               &               &               &               &               &               &               &               &               &               &       (.29)   \\
Scientific Veneer $\times$ Pro AI&               &               &               &               &               &               &               &               &               &               &         .29   \\
                    &               &               &               &               &               &               &               &               &               &               &       (.53)   \\
\hline
Observations        &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &       1,984   &         992   \\
\(R^{2}\)           &        .015   &        .024   &       .0034   &        .047   &        -.12   &        -.39   &        .041   &        -1.1   &        .016   &        -1.1   &         .84   \\
\end{tabular}

